Bridging MDE and AI: A Systematic Review of Domain-Specific Languages and Model-Driven Practices in AI Software Systems Engineering

Background:Technical systems are growing in complexity with more components and functions across various disciplines. Model-Driven Engineering (MDE) helps manage this complexity by using models as key artifacts. Domain-Specific Languages (DSL) supported by MDE facilitate modeling. As data generation in product development increases, there's a growing demand for AI algorithms, which can be challenging to implement. Integrating AI algorithms with DSL and MDE can streamline this process. Objective:This study aims to investigate the existing model-driven approaches relying on DSL in support of the engineering of AI software systems to sharpen future research further and define the current state of the art. Method:We conducted a Systemic Literature Review (SLR), collecting papers from five major databases resulting in 1335 candidate studies, eventually retaining 18 primary studies. Each primary study will be evaluated and discussed with respect to the adoption of MDE principles and practices and the phases of AI development support aligned with the stages of the CRISP-DM methodology. Results:The study's findings show that language workbenches are of paramount importance in dealing with all aspects of modeling language development and are leveraged to define DSL explicitly addressing AI concerns. The most prominent AI-related concerns are training and modeling of the AI algorithm, while minor emphasis is given to the time-consuming preparation of the data. Early project phases that support interdisciplinary communication of requirements, e.g., CRISP-DM Business Understanding phase, are rarely reflected. Conclusion:The study found that the use of MDE for AI is still in its early stages, and there is no single tool or method that is widely used. Additionally, current approaches tend to focus on specific stages of development rather than providing support for the entire development process.

==> tables/final_results.tex <==
\begin{table}
\centering
\begin{footnotesize}
\caption{List of selected publications with type of publication incl. snowballing results.}
\label{tab:final_papers}
\begin{tabularx}{\linewidth}{|l|r|l|X|} 
\hline
\textbf{Item Type} & \textbf{Year} & \textbf{Author} & \textbf{Title} \\ 
\hline
Conference Paper & 2020 & \cite{al-azzoni_model_2020} & Model Driven Approach for Neural Networks \\ 
\hline
Conference Paper & 2023 & \cite{bergerEVOALDomainSpecificLanguageBased2023} & EVOAL: A domain-specific language-based approach to optimisation \\ 
\hline
Conference Paper & 2019 &  \cite{bhattacharjee_stratum_2019} & STRATUM: A BigData-as-a-Service for Lifecycle Management of IoT Analytics Applications \\ 
\hline
% Journal Article & 2014 & \cite{breuker_towards_2014} & Towards Model-Driven Engineering for Big Data Analytics–An Exploratory Analysis of Domain-Specific Languages for Machine Learning \\ 
% \hline
Journal Article & 2020 & \cite{de_la_vega_lavoisier_2020} & Lavoisier: A DSL for increasing the level of abstraction of data selection and formatting in data mining \\
\hline
Conference Paper & 2021 & \cite{delineGlindaSupportingData2021} & Glinda: Supporting data science with live programming, GUIs and a domain-specific language \\ 
\hline
Journal Article & 2022 & \cite{giner-miguelez_domain-specific_2022} & A domain-specific language for describing machine learning dataset \\ 
\hline
Conference Paper & 2017 & \cite{hartmann_next_2017} & The next Evolution of MDE: A Seamless Integration of Machine Learning into Domain Modeling \\ 
\hline
Conference Paper & 2019 & \cite{hartmann_meta-modelling_2019} & Meta-Modelling Meta-Learning \\ 
\hline
Conference Paper & 2019 & \cite{hartsell_model-based_2019} & Model-based design for CPS with learning-enabled components \\
\hline
Conference Paper & 2019 & \cite{koseler_realization_2019} & Realization of a Machine Learning Domain Specific Modeling Language: A Baseball Analytics Case Study \\ 
\hline
Conference Paper & 2019 & \cite{kusmenko_engineering_2019} & On the Engineering of AI-Powered Systems \\
\hline
Journal Article & 2021 & \cite{meacham_adaptivesystems_2021} & AdaptiveSystems: An Integrated Framework for Adaptive Systems Design and Development Using MPS JetBrains Domain-Specific Modeling Environment \\ 
\hline
Conference Paper & 2022 & \cite{melchor_model-driven_2022} & A Model-Driven Approach for Systematic Reproducibility and Replicability of Data Science Projects \\
\hline
Journal Article & 2021 & \cite{moin_model-driven_2022} & A Model-Driven Engineering Approach to Machine Learning and Software Modeling \\ 
\hline
Journal Article & 2023 & \cite{pinedaRADENNDomainSpecificLanguage2023} & RADENN: A Domain-Specific Language for the Rapid Development of Neural Networks \\ 
\hline
Journal Article & 2022 & \cite{morales_towards_2022} & Towards a DSL for AI Engineering Process Modeling \\ 
\hline
Journal Article & 2014 & \cite{breuker_towards_2014} & Towards Model-Driven Engineering for Big Data Analytics–An Exploratory Analysis of Domain-Specific Languages for Machine Learning \\ 
\hline
Conference Article & 2023 & \cite{radlerCodeGenerationMachine2023} & Code Generation for Machine Learning using Model-Driven Engineering and SysML \\ 
\hline
Conference Paper & 2021 & \cite{ries_mde_2021} & An MDE Method for Improving Deep Learning Dataset Requirements Engineering using Alloy and UML \\ 
\hline
Conference Paper & 2020 & \cite{zucker_arbiter_2020} & Arbiter: A Domain-Specific Language for Ethical Machine Learning \\ 
\hline
% Conference Paper & 2022 & \cite{guizzardi_towards_2022} & Towards Integrated Model-Driven Engineering Approach to
%   Business Intelligence \\
% \hline
\end{tabularx}
\end{footnotesize}
\end{table}

==> temp-remove/PLM-stuff.tex <==
\luca{PLM-related discussion is too long imho. I do not see a particular reason to have such a specific discussion/presentation in the introduction. It makes sense in the result or discussion section.}
A particular example of a case-specific data-driven engineering application in practice is using product lifecycle management (PLM) data to improve production performance or generate valuable information for the design or production to make informed decisions.
\del{PLM is a concept that enables the management of data and processes from the inception and development to the manufacture, maintenance, and disposal of a product during its product lifecycle~\cite{stark_plm_2016}. 
For example, PLM data can be enriched during engineering (computer-aided design (CAD), computer-aided manufacturing (CAM)) and production via interfaces to production-related machines, such as a lathe or a robot, as shown in an example shop floor in Figure~\ref{fig:prodpic}, which is being implemented in the pilot factory of the Vienna University of Technology~\cite{hennig_tu_2019}.}
\begin{figure}
    \centering
    \includegraphics[width=0.75\textwidth]{figures/prod.jpeg}
    \caption{An example of a production hall where data is collected during the production of turned parts.}
    \label{fig:prodpic}
\end{figure}
%\luca{The same comment of the previous paragraph applies here. It seems we are narrowing the scope of the SLR by introducing these details in the introduction. However, it is not reflected in the search string. So this is something that goes in the discussion. Again, the problem is, do we catch these papers with the search strings?}
\del{Although PLM data might be collected during manufacturing, the potential and opportunities of AI to generate valuable insights are not entirely reflected in the industry due to a lack of knowledge for the implementation and the missing number of employees on the market~\cite{anaconda_state_2022,radler_survey_2022}.}
%\luca{if the following paragraph refers again to PLM, it has to be moved as well.}
\luca{if it relates to PLM only then I would remove it from the intro.}
\del{With \del{the integration of} MDE for AI, a foundation for non-programmers to define AI tasks by formalizing knowledge is given.
Additionally, AI experts might rely on AI task formalization that can be transformed into (partly) executable code by facilitating model transformation.
Moreover, knowledge representation of various domains can be integrated, allowing \chg{to interchange}{share} the understanding and reduce the shortcomings of undocumented work.
Further, semantic connections of data attributes from the PLM can be drawn, allowing to trace origination, data relations, and reuse of specifications.}

==> temp-remove/attribute_comparison.tex <==
In this section, the comparison of the assessed approaches with respect to the various dimensions is depicted.
\subsubsection{Meta-Models}
12 of the 18 approaches are depicting a meta-model.

In \cite{al-azzoni_model_2020}, EMF based meta-model is depicted with special focus on the dataset and multi-layer perception (MLP) NN. Various enums are defined to specify valid values, e.g. dataset normalization types.
In \cite{bhattacharjee_stratum_2019}, two meta-models are presented on the referenced artifacts. First, a main meta-model of the learning plattform and second, a meta-model of the ML algorithms.
In \cite{de_la_vega_lavoisier_2020}, an Ecore based meta-model is defined with focus on the filtering and description of various datasets.
In \cite{giner-miguelez_domain-specific_2022}, three meta-models are described 1) metadata model, 2) composition model and 3) provenance and social concerns model.
In \cite{hartmann_next_2017}, a meta-meta model integration is depicted since the approach is in a higher-level of modeling integrated.
In \cite{hartmann_meta-modelling_2019}, a conceptual meta-model for machine learning as well as for meta-learning is depicted. The meta-model for ML contains a definition for dataset meta data as well as a definition for the learning algorithm with hyeper-parameters.
In \cite{hartsell_model-based_2019}, the meta-model is based on existing meta-model libraries: SEAM, DeepForge and ROSMOD.
In \cite{koseler_realization_2019}, the meta-model is represented using SysML in the modeling framework Papyrus, which is also based on Ecore.
%In \cite{kusmenko_engineering_2019}, 
In \cite{melchor_model-driven_2022}, various metamodel are depicted using means of EMF, which is basically Ecore\footnote{\url{https://eclipse.org/modeling/emf/}}.
In \cite{moin_model-driven_2022}, an Ecore meta-model is presented that is generated out of the Xtext grammar.
In \cite{taibi_towards_2022}, the entire meta-model is depicted in an unknown modeling language but with a fashion like Ecore.
In \cite{ries_mde_2021}, a Ecore based meta-model is defined with five main elements, each described textually.



\subsubsection{Abstract Syntax}
13 of the 18 approaches are depicting an abstract syntax.

In \cite{bhattacharjee_stratum_2019}, the abstract syntax is captured in multiple metamodels, but not explicitly mentioned. 
In \cite{breuker_towards_2014}, the abstract syntax is depicted in a figure with an entity relationship notation.
In \cite{de_la_vega_lavoisier_2020}, the abstract syntax is defined using Ecore modeling. It characterizes the main composition of the dataset with various filters.
In \cite{giner-miguelez_domain-specific_2022}, the abstract syntax is implicitly defined in the meta-models and textually described.
In \cite{hartmann_next_2017}, the abstract syntax is implicitly defined by the meta-meta model and the underlying language principles.
In \cite{hartmann_meta-modelling_2019}, the abstract syntax is implicitly with the previous approach in \cite{hartmann_next_2017} given.
In \cite{hartsell_model-based_2019}, block diagram models from SysML are used and therefore, the abstract syntax is aligned with SysML.
In \cite{koseler_realization_2019}, the abstract syntax is given in the original concept \cite{breuker_towards_2014}.
In \cite{kusmenko_engineering_2019}, the abstract syntax tree (AST) is adapted internally using the MontiCore's language aggregation concept \cite{rumpe_monticore_2017}.
In \cite{meacham_adaptivesystems_2021}, an abstract syntax tree is used to define the language. However, the details are not entirely published and artifacts are not available.
In \cite{melchor_model-driven_2022}, is defined using means of the Eclipse Modeling Framework (EMF). 
In \cite{moin_model-driven_2022}, the abstract syntax is defined in the grammar of Xtext.
In \cite{taibi_towards_2022}, the abstract syntax is implicitly defined with the meta-model on Sirius web.

\subsubsection{Concrete Syntax}
15 of the 18 approaches are depicting an concrete syntax.

In \cite{al-azzoni_model_2020}, the concrete syntax is realized using EMF modeling syntax.
In \cite{bhattacharjee_stratum_2019}, the concrete syntax is defined by the underlying modeling framework WebGME.
In \cite{de_la_vega_lavoisier_2020}, a xtext grammar aligned textual syntax is specified due to the author's believe that the definition of the datasets is faster using text than graphical modeling.
In \cite{dethlefs_define_2017}, a text based syntax based on Python using libraries such as numpy etc. is depicted.
In \cite{giner-miguelez_domain-specific_2022}, a text based concrete syntax using visual studio editor with a plugin is described.
In \cite{hartmann_next_2017}, an Emfatic inspired textual modeling language is defined.
In \cite{hartmann_meta-modelling_2019}, an Emfactic inspired textual syntax is given.
In \cite{hartsell_model-based_2019}, WebGME graphical modeling is applied.
In \cite{koseler_realization_2019}, the concrete syntax uses Papyrus graphical modeling.
In \cite{kusmenko_engineering_2019}, a concrete textual syntax is used to describe AI concerns while a graphical approach is used for the C\&C architecture.
In \cite{meacham_adaptivesystems_2021}, a textual syntax using the MPS framework is depicted.
In \cite{moin_model-driven_2022} an Xtext based model editor in EMF with concrete textual syntax is presented.
In \cite{taibi_towards_2022}, the graphical modeling environment Sirius Web is used.
In \cite{ries_mde_2021}, a Sirius framework based UML class diagram syntax is used.
In \cite{zucker_arbiter_2020}, a SQL-like textual editor is used.


\subsubsection{Arbitrary Constraints}
7 of the 18approaches are depicting arbitrary constraints.


In \cite{al-azzoni_model_2020}, the constraints are formalized using Epsilon Validation Language (EVL).
In \cite{bhattacharjee_stratum_2019}, the definition of constraints is built on the underlying principles of WebGME. 
In \cite{hartsell_model-based_2019}, constraints are given due to the system architecture model based on SysML Internal Block Diagram that allow to specify constraints.
In \cite{koseler_realization_2019}, constraints are given due to the underlying SysML.
%In \cite{kusmenko_engineering_2019}, ???
In \cite{melchor_model-driven_2022}, means of OCL expression constraints is used to limit the input ports. It is still unclear whether constraints can be modeled in the instantiation of the metamodel.
In \cite{ries_mde_2021} a textual predicate is allowed that conforms to the Alloy language as a textual expression.
In \cite{zucker_arbiter_2020}, relational operators with \textit{'and'} and \textit{'or'} operators are used to define constraints.



\subsubsection{Model Transformation}
12 of the 18 approaches are depicting model transformations.

In \cite{al-azzoni_model_2020}, the Epsilon Generation Language (EGL) is used with templates to define the model transformation to generate Java code.
In \cite{bhattacharjee_stratum_2019}, code generation capabilities of WebGME are used and extended with templates for each of the subtask.
In \cite{de_la_vega_lavoisier_2020}, the dataset description is transformed into tabular datastes using low-level data transformation operations. The datasets are then usable in data mining algorithms.
In \cite{hartmann_next_2017}, the framework GreyCat that is built on Kevoree Modeling Framework provides code generation toolsets to build object-oriented applications.
In \cite{hartmann_meta-modelling_2019}, it is said that code generators generate the machine learning code. Details are missing.
In \cite{hartsell_model-based_2019}, the toolchain configures an embedded Jupyter notebook to execute the model.
In \cite{koseler_realization_2019}, C# code is generated using means of Epsilon model transformation.
In \cite{kusmenko_engineering_2019}, MontiAnna2X code generator is used to generate MxNet, Caffe2 or Tensorflow code.
In \cite{meacham_adaptivesystems_2021}, means of MPS language are used to generate Java code.
In \cite{moin_model-driven_2022}, means of Java and Xtend are used to generate Python code.
In \cite{ries_mde_2021}, model2text transformation is used to allow the completion of formal specification using Alloy Analyzer.


\subsubsection{Frameworks (Methods \& Tools)}
18 of the 18 approaches are depicting frameworks such as methods and tools.

In \cite{al-azzoni_model_2020}, EMF, EGL and EVL is used for the modeling.
In \cite{bhattacharjee_stratum_2019}, WebGME is used as foundation.
In \cite{breuker_towards_2014}, a concept is depicted without featuring specific frameworks.
In \cite{guizzardi_towards_2022}, no frameworks and tools are presented since it is a concept.
In \cite{de_la_vega_lavoisier_2020}, xtext for the grammar and ecore for the definition of the metamodel.
In \cite{dethlefs_define_2017}, Python and its libraries are used in a fluent interface language extension.
In \cite{giner-miguelez_domain-specific_2022}, based on visual studio with a plugin and the textual low-code language is based on Langium.   
In \cite{hartmann_next_2017}, GreyCat.
In \cite{hartmann_meta-modelling_2019}, Sirius Web.
In \cite{hartsell_model-based_2019}, SysML, SEAM, DeepForge, ROSMOD, Jupyter Notebook WebGME, Goal Structuring Notation (GSN)
In \cite{koseler_realization_2019}, Papyrus, Epsilon.
In \cite{kusmenko_engineering_2019}, MontiCore Workbench.
In \cite{meacham_adaptivesystems_2021}, Jetbrains MPS.
In \cite{melchor_model-driven_2022}, Python.
In \cite{moin_model-driven_2022}, Xtext, XTend, ThingML, Papyrus.
In \cite{taibi_towards_2022}, Sirius Web, 
In \cite{ries_mde_2021}, Sirius, Alloy, BPMN, XTend, KodKod (SAT-based constraint solver)
In \cite{zucker_arbiter_2020}, Python, SQL?


\subsubsection{Requirements Modeling}
4 of the 18 approaches are depicting requirements modeling.

In \cite{hartsell_model-based_2019}, a Goal Structuring Notation (GSN) approach is used to define and structure requirements.
In \cite{taibi_towards_2022}, the meta-model reflects means to model requirements.
In \cite{ries_mde_2021}, the entire paper deals with the detailed modeling of requirements.
In \cite{zucker_arbiter_2020}, requirements on the ethical machine learning can be formalized, such as protecting the classes 'race' or 'age'.


\subsubsection{Business Understanding}
4 of the 18 approaches are depicting business understanding.

In \cite{guizzardi_towards_2022}, the concept to store the busines understanding separate from data in a custom application layer model (referred to as OLAP-VIZ model) is proposed.
In \cite{hartsell_model-based_2019}, the business understanding is fostered due to the requirements modeling and the component modeling using SysML.
In \cite{taibi_towards_2022}, with the integration of \textit{Roles}, business relevant information are modeled, leading to an increased business understanding.


\subsubsection{Data Understanding}
9 of the 18 approaches are depicting data understanding.

In \cite{breuker_towards_2014}, the data understanding is fostered by describing the datasets with data interrelations (as of the abstract syntax).
In \cite{guizzardi_towards_2022}, conceptually, the data understanding is fostered by mapping data source values to the ETL and describe the specification of the data warehouse stored data in a model.
In \cite{de_la_vega_lavoisier_2020}, the contextualization of the dataset properties enable to improve the data understanding by implicitely apply rules on how to select data.
In \cite{giner-miguelez_domain-specific_2022}, With the detailed description of a dataset, the data composition and overall understanding is fostered.
In \cite{hartmann_next_2017}, the enrichment of properties on a metamodel level is enabled that contributes to further description of the properties and therefore, data understanding. Additionally, the interconnection of the data properties is highlighted by the underlying principle. Still, the description of the attributes itself is not so rich, leading to no support in the understanding of a single property and its origin.
In \cite{hartmann_meta-modelling_2019}, same as for \cite{hartmann_next_2017}.
In \cite{koseler_realization_2019}, data understanding is fostered due to the graphical representation of the input data and the composition of the variables.
In \cite{melchor_model-driven_2022}, data understanding is fostered by describing data attributes such as the data type. Additionally, the type of ML algorithm is described, allowing to reproduce a ML project.
In \cite{ries_mde_2021}, the advanced requirements modeling allows to understand certain data better.

\subsubsection{Data Ingestion}
12 of the 18 approaches are depicting data ingestion.

In \cite{al-azzoni_model_2020}, the loading of text based datasets is defined with a delimiter, filepath etc. However, the integration of other data structures, such as SQL is not intended.
In \cite{bhattacharjee_stratum_2019}, the loading of data from various edge devices is presented using technologies such as RabittMQ or Kafka. 
In \cite{de_la_vega_lavoisier_2020}, the loading of the dataset is described by specifying the name and path of the file or SQL server in combination with sql selection scripts.
In \cite{dethlefs_define_2017}, data ingestion is realized by using the Python dataset methods implemented in specific libraries.
In \cite{hartsell_model-based_2019}, the data is generated and collected with simulation or execution instances. The data is stored on the fileserver.
In \cite{kusmenko_engineering_2019}, data loading is provided with tagging schemas for EMADL ports.
In \cite{meacham_adaptivesystems_2021}, a path with the input dataset is specified at the beginning of each ML implementation.
In \cite{melchor_model-driven_2022}, the file type ,e.g. CSV or JSON is depicted with a data store uri.
In \cite{moin_model-driven_2022}, two approaches are given, first an blackbox approach, where the ML model is imported from a pickle and second, the paths or URLs of the dataset(s) are passed to the training, validation and testing of the algorithm.
In \cite{taibi_towards_2022}, the loading of data from various sources such as SQL servers is depicted in a sample as well as in the meta-model.
In \cite{zucker_arbiter_2020}, the origin of the data can be specified with a file name/path.

\subsubsection{Feature Preparation}
8 of the 18 approaches are depicting feature preparation.

In \cite{al-azzoni_model_2020}, features of the loaded dataset can be normalized. However, more advanced data pre-processing steps are not defined in the meta-model.
In \cite{bhattacharjee_stratum_2019}, the feature preparation is defined in the metamodel. Still, details on the specific methods are missing.
In \cite{dethlefs_define_2017}, wrappers around Python libraries are created that pre-process datasets.
%In \cite{kusmenko_engineering_2019}, ???
In \cite{melchor_model-driven_2022}, data operations can be applied to a specific data set.
In \cite{moin_model-driven_2022}, each state allows to execute functions. The keyword DA\_Preprocess is used to apply data praparation functions to a specific dataset.
In \cite{taibi_towards_2022}, features can be prepared with specific \textit{feature extraction techniques}, data can be transformed with data engineering techniques, e.g. \textit{Regression substituion}.

\subsubsection{Model Training}
14 of the 18 approaches are depicting model training.

In \cite{al-azzoni_model_2020}, the training is defined using MLP description, e.g. learning rules like Backpropagation etc. Further details on other hyper-parameters or the facilitation of the output is not given.
In \cite{bhattacharjee_stratum_2019}, the model training is defined using NN methods that are pre-defined.
In \cite{breuker_towards_2014}, the model training is given due to an assignment for each variable whether it is an observed, random or just an variable. 
In \cite{dethlefs_define_2017}, the training algorithm is specified using a \textit{modelString} with the name of the algorithm and various hyper-parameters.
In \cite{hartmann_next_2017}, various algorithm models can be used with specific learning and output attributes.
In \cite{hartmann_meta-modelling_2019}, same as for \cite{hartmann_next_2017}.
In \cite{hartsell_model-based_2019}, the training defined in a experiment model. The details of the implementation can be found in the Jupyter notebooks.
In \cite{koseler_realization_2019}, the inference model for training is graphically defined. The data for the training is passed by the generated code. Details on hyper-parameter tuning are not given.
In \cite{kusmenko_engineering_2019}, the training of NN is given with possibilities to specify layers and connections.
In \cite{meacham_adaptivesystems_2021}, the algorithm (referred to as Approach) is specified with various hyper-parameters, e.g. Random Forst Cross Validation Folds.
In \cite{melchor_model-driven_2022}, the algorithm type with task type can be described.
In \cite{moin_model-driven_2022}, the state keyword DA\_Train is used to lead to training and the DA\_Predict to apply the trained model to certain data.
In \cite{taibi_towards_2022}, hyper-parameters and performance criteria can be specified for each AI model.

\subsubsection{Metrics/Evaluation}
5 of the 18 approaches are depicting metrics or evaluations.

In \cite{bhattacharjee_stratum_2019}, metrics are integrated in the meta-model and can be applied on the training output.
In \cite{dethlefs_define_2017}, evaluation metrics such as \textit{accuracy} measurement can be added to the training model definition.
In \cite{hartsell_model-based_2019}, metrics are applied in the Jupyter notebooks.
In \cite{kusmenko_engineering_2019}, the metrics of the evaluation is selected using the name of the metrics, e.g. Mean squared error (mse)
In \cite{moin_model-driven_2022}, basic metrics such as Mean Absolute Error (MAE) or Mean Squareed Error (MSE) can be applied among other to the algorithms, such as regression algorithms.

\subsection{Artifacts Available and Domain of application}
In \cite{al-azzoni_model_2020}, the artifacts are presented in the paper. However, a comprehensive replicate of the artifacts of the evaluation are not given. The evaluation is based on a diabetes dataset.
In \cite{bhattacharjee_stratum_2019}, artifacts are stored on github with the entire sample and additional information such as meta-model graphs. The purpose of the MDE approach originates in the domain of IoT devices.
In \cite{breuker_towards_2014}, the artifacts are not available since it is an early concept. Additionally, the domain of application can be categorized as any.
In \cite{guizzardi_towards_2022}, no artifacts are available since it is a concept only.
In \cite{de_la_vega_lavoisier_2020}, the artifacts of the lavoisier language as well as the evaluation is available on github.
In \cite{dethlefs_define_2017}, no artifacts are available to prove the work. As of the fluent language design, it is applicable to any domain.
In \cite{giner-miguelez_domain-specific_2022}, the plugin and source code as well as a proof video is available online.
In \cite{hartmann_next_2017}, the experiment as well as the dsl is available online.
In \cite{hartmann_meta-modelling_2019}, no artifacts are available since the approach is more conceptually depicted.
In \cite{hartsell_model-based_2019}, most of the artifacts are available in a test-bed online. However, the machine learning part could not be varified.
In \cite{koseler_realization_2019}, the entire Papyrus model with all artifacts, such as the data pre-processing Jupyter notebook, are available online.
In \cite{kusmenko_engineering_2019}, the entire code of the MontiCore family is available online.
In \cite{meacham_adaptivesystems_2021}, artifacts are not referenced. The problem domain was adaptive virtual learning environments.
In \cite{melchor_model-driven_2022}, artifacts are given in a github repository. The domain of application seem to be any.
In \cite{moin_model-driven_2022}, the entire code of the so-called ML-Quadrat toolbox is available on github.
In \cite{taibi_towards_2022}, the meta-model is available as figures in an extended paper artifact. The implementation of the model could not be found online. The domain of application is any.
In \cite{ries_mde_2021}, the entire toolset is available as online resources.
In \cite{zucker_arbiter_2020}, the code is hosted on github.

==> temp-remove/intro_old.tex <==
\section{Introduction}\label{sec:introduction}
\karo{Sollten wir zu Beginn noch ein konkretes Beispiel einbauen? Dieses würde sicherlich helfen das Setting und die Dimension des Problems noch verständlicher zu machen. Gegebenenfalls auch die Unterschiede zwischen den einzelnen Begriffen, z.B. MDE, MBSE (kann aber auch daran liegen, dass ich mich gerade erst in die Materie einlesen vll ist das eh klar)}

\marginpar{Evolving System Complexity}Engineered systems are getting more complex due to the increasing number of components and functions and the involvement of several disciplines \citep{beihoff_world_2014}.
To manage this complexity, the integration of model-driven engineering (MDE) and model-based systems engineering (MBSE) has proven beneficial \cite{shinde_review_2018,dogan_machine_2021}.
\marginpar{MDE}MBSE aims to support the development of engineered systems by providing and maintaining information for the development using models rather than documents \cite{henderson_value_2021}.
Models are shared among stakeholders and manipulated by Computer-Aided Software Engineering (CASE) tools, aiming at the highest possible degree of automation (e.g., via model transformations).
Consequently, MBSE techniques allow for making informed decisions based on formalized/modeled data.
However, MBSE techniques lack the means to gather sufficient knowledge from more extensive data, e.g., Big Data.
\marginpar{AI}In this respect, means of artificial intelligence (AI) and its sub-disciplines, namely machine learning (ML) and deep learning (DL), are beneficial to exploit the information hidden in data \cite{provost_data_2013}.
The integration of data-driven methods to support engineering tasks has recently been defined as data-driven engineering \cite{trauer_data-driven_2020} and has been proven to be beneficial in several engineering areas such as manufacturing \cite{dogan_machine_2021}, aerospace industry \cite{brunton_data-driven_2021} or other industrial applications \cite{bertolini_machine_2021,fahle_systematic_2020,sarker_machine_2021}.
\marginpar{Potential not reflected}Still, the potential and opportunities of AI are not entirely reflected in the industry due to a lack of knowledge for the implementation, and the missing number of employees on the market \cite{anaconda_state_2022,radler_survey_2022}.
\marginpar{Integration of AI and MDE challenge}The need for experts to implement data-driven solutions will further increase due to the demand to integrate artificial intelligence in existing methods such as MBSE \cite{davey_systems_2022}.
Concerning this, recently, a series of workshops on artificial intelligence and model-driven engineering has begun, presenting the use of model-driven engineering (MDE) techniques for the definition of AI and AI support for MDE \cite{burgueno_mde_2021-1,burgueno_mde_2021,burgueno_guest_2022}.
Still, the current state of practice and state of the art is not elaborated regarding MDE approaches that support the implementation of AI.

\marginpar{RQ and Contribution} Concerning this, the following research question drives this paper:
\textbf{What is the current state of the art for model-driven engineering with extensions to formalize artificial intelligence?}
With respect to this, a systematic literature review according to the guidelines set out by \cite{kitchenham_systematic_2013} is conducted to gather and assess existing literature \cite
{petersen_guidelines_2015}.
Particularly, the focus of this work is to investigate the state-of-the-art for model-driven engineering approaches that enable the modeling of artificial intelligence.
Since the workshop on MDE for AI and the author's known publications are very recently published, the number of MBSE publications seems small; therefore, the broader term MDE is further used in this SLR.

\marginpar{reminder of the paper}The rest of the paper is organized as follows. Section \ref{sec:background} provides background on the used terms such as model-driven engineering and artificial intelligence.
Section \ref{sec:method} introduces the protocol adopted to perform the SLR, focusing on reproducibility.
Section \ref{sec:results} presents the approaches aligned with the data extraction strategy of the SLR protocol in Section \ref{sec:method}.
Section \ref{sec:discussion} discusses the key findings, depicts implications and future research, assesses the quality and limitations of the current SLR using threats to validity analysis and answers the research questions.
Section \ref{sec:conclusion} summarizes the paper.

==> temp-remove/paper_summary.tex <==
\section{\cite{al-azzoni_model_2020}}
In this approach, a EMF meta-model is shown that enables to load a Dataset, describe a Multi-Layer Perception algorithm and train the data.

The approach is yet not generic applicable for multiple algorithms.
The approach is based on Eclipse modeling Framework (EMF).
The meta-model shows various aspects such as description of the problem, dataset details and training parameters.
The concrete syntax is defined as EMF and therefore both graphical and textual is possible.
The abstract syntax is not explicitly defined.
Constraints are possible due to the underlying principle of EMF
Model transformation are integrated using templates for Ecplise Epsilon code generation.

The approach does not contribute to the business understanding data understanding.
The data ingestion is depicted in the meta-model using dataset description.
Feature preparation is given due to normalization methods. However, the sequential execution of multiple preprocessing operations is not available.
The model training is specified by a fixed algorithm. Still, further NN models shall be integrated in future work.
The approach is validated using Pima Indians Diabetes dataset.


\section{\cite{bhattacharjee_stratum_2019}}
The paper provides a model-driven tool called STRATUM to deal with the lifecycle of intelligent components, from design-related concerns (e.g. modeling the pipeline of a ML algorithm), the access to data streams, the allocation to a properly dimensioned cloud-based execution platform, the monitoring of QoS of the overall system. STRATUM is built on top of the WebGME (meta)modeling framework.

Although stratum is able to formalize knowledge for machine learning approaches, the level of detail is sometimes low, e.g. for data ingestion pre-processing or data understanding.
The approach does not formalize knowledge on the business and thus, does not foster the understanding.
The data understanding is not explicitly given with respect to the measurement dimensions.

\section{\cite{breuker_towards_2014}}
see Koseler


\section{\cite{guizzardi_towards_2022}}
This paper introduces a blueprint of a MDE method to describe BI tasks.
The aimed approach reflects business and data understanding.
Still, the concept is in a quite early state and therefore, no detailed assessment can be made.

The authors state that a comprehensive a review on MDE for BI is necessary. As of now: No review found on the internet

\section{\cite{de_la_vega_lavoisier_2020}}
The approach shows a DSL that allows to model data preparation on a high-level.
The approach introduces a conceptual model that can be viewed as a meta-model.
The syntax is aligned with SQL syntax and textually applied.
Still, an intermediate domain model using graphical modeling is integrated.
Constraints can be defined using if/else programming logic.

The approach reflects data understanding by integrating a object oriented domain model using ecore.
In the paper, the the loading of data is not detailed. In the artifact repository, there is a loading command in the generated file. However, we cannot assess whether it is modeled or not.


\section{\cite{dethlefs_define_2017}}
The approach shows a fluent interface DSL that allows to define DeepLearning approaches including preprocessing, modeling and evaluation.
The approach allows to formulate a DeepLearning approach with less code than usual Python implementation.

From an language perspective, only the concrete syntax as well as the model transformation is specified.
The representation of the data & business understanding is not given
Data ingestion with feature preparation is applied using an approach that is similar to programming.
Model training is the most prominent part with hyper-parameters.
Unfortunately, no artifacts referenced for replication.
The approach seem to help programmers but neither communication nor the explainability or understanding.


\section{\cite{giner-miguelez_domain-specific_2022}}
In this approach, a model-based description of machine learning datasets is introduced.
The DSL focuses on the description of metadata, data attributes with statistical features as well as provenance and social concerns.
In future research, the authors aim to adapt the DSL to describe ML models and other parts of the ML pipeline.
Consequently, the data understanding is fostered while the other dimensions are future work.

Shortcoming: The approach does not reflect the data source in detail, which might lead to miss-interpretation and shortcomings in the description of potential biases. Additionally, the gathering of data is described as full-text that lead to missing connection to systems engineering processes. Finally, the dataset description focuses on human datasets (e.g. Demographic aspects). Therefore, the integration in engineering processes with machine only datasets is limited.


\section{\cite{hartmann_next_2017}}
In~\cite{hartmann_next_2017}, an approach applying so-called microlearning units, which are small, reusable, changeable and independently computable learning units, is depicted. Due to the high entanglement of learning units and domain knowledge, Hartmann proposes to weave the learning units into domain modeling. The modeling of the approach is conducted in the open source framework GreyCat, an extension of the Kevoree modeling framework KMF~\citep{fouquet_eclipse_2012}. The KMF is similar to the EMF, which is the basis of the open source modeling framework Papyrus\footnote{\url{https://www.eclipse.org/papyrus/}}. Concerning the referenced repository on github\footnote{\url{https://github.com/kevoree-modeling}}, Kevoree modeling is not maintained anymore. 
The depicted approach of~\cite{hartmann_next_2017} extends the meta-meta model of GreyCat with properties to describe what should be learned, how (algorithm, parameters) and the from what (attributes, relations,...). The extension defines a new grammar for the textual modeling language. To connect the grammar with learning units, GreyCat uses patterns to map the code generator from the modeling to the templates. 
The approach does not introduce means of requirements definition.
The business understanding is not fostered since other domain knowledge is not formalized. Still, the approach promises to allow the weaving into other formalization due to the underlying principles (Section III-D)
The data understanding is given by the underlying principle and the modeling of interconnections of the data.
Data ingestion is not present since the origin of data sources is not formalized.
Feature preparation is not explicitly presented.
The model training is given by selecting an algorithm with hyper-parameters.
Metrics are not mentioned.
The approach is validated using a Smart Meter sample from the IoT domain.

\section{\cite{hartmann_meta-modelling_2019}}
\cite{hartmann_meta-modelling_2019} builds upon \cite{hartmann_next_2017} and describes the integration of meta-learning using model-based approaches in Greycat.
In the approach, the metamodel for machine learning in \cite{hartmann_next_2017} is extended towards metamodeling.
Apart from that, no further contribution to the SLR.
The findings are not evaluated and therefore, no domain is said. Still, the IoT/CPS domain seem to match.

\section{\cite{hartsell_model-based_2019}}
The given approach shows a comprehensive modeling environment for learning enabled components in the context of CPS development.
The artifacts are online available\footnote{\url{https://modelbasedassurance.org/}}
Either online or in the publication, all aspects of MDE are described or illustrated.
The approach allows to define requirements by defining goals and potential solutions.
With the integration of CPS modeling aspects, the business understanding is fostered.
However, the description of the data understanding has some shortcomings.
Also the feature preparation is not described in detail.
The approach focuses on the domain of CPS development.

\section{\cite{koseler_realization_2019}}
The basic concept of this work originates from \cite{breuker_towards_2014}.
The approach of \cite{breuker_towards_2014} neither is implemented nor validated and thus, \cite{koseler_realization_2019} adapted the approach with an improved an more comprehensive syntax and concept.

The approach is based on a Papyrus profile that are used to define the metamodel.
However, the approach does not contribute to a better understanding of the business or data understanding since the entire dataset is embedded in the UML file as encoded values. To do this, data pre-processing is externally applied.
The abstract syntax is defined in \cite{breuker_towards_2014} and the concrete syntax is defined by Eclipse modeling framework.
The data understanding is partly given due to the connection between various variables. However, it could be more improved with additional insights regarding origin or data distribution.
The data ingestion is not given since the data is directly embedded in the UML model. Therefore, other sources than the case study cannot be readily integrated.
Entire testing code is public available.
The actual domain is from the sport analytics, still other domains seem to be reasonable.

\section{\cite{kusmenko_engineering_2019}}
In~\cite{kusmenko_engineering_2019}, an approach describing machine learning using modeling is presented. The applied approach is based on the MontiAnna framework, an umbrella term for multiple frameworks and code generators. The frameworks are intended to define deep artificial neural networks, e.g. CNN. Textual modeling is applied to define the AI viewpoint and graphical modeling to model the components\&connectors, e.g. CPS interface. The given approach is intended to be used for artificial neural networks and particularly enables to the formalization of the machine learning from the input over the flow by using ports and connections until the learning dimensions and related output. With the different levels of integration, architectural and implementation aspects are depicted and the generators enable the generation of Python code for the training and C++ code for embedding the learned model. The approach seems highly correlated to programming but is supported by modeling approaches. The approach's scope limitation is on artificial neural networks and a set of pre-implemented algorithms. 

From an language perspective, all dimensions are reflected either in the publication or in one of the other by Kusmenko.
The approach is heavily based on the definition of AI and therefore, do not support data or business understanding and also the interdisciplinary communication is little fostered.

\section{\cite{meacham_adaptivesystems_2021}}
This approach introduces a set of DSLs to describe adaptive systems in the design phase while integrating machine learning.
The concept shows how to load, store a model.
Previous publications deal with the training of a model.

The approach does not introduce a metamodel, but an abstract syntax tree.
The implementation using a textual modeling environment, namely Jetbrains MPS, is presented.
The model is transformed into executable code.

The approach does not support business or data understanding.
The data preparation is shown in a previous work [ref 10 in the paper].
Same as for the data prepraration, the model training is depicted in ref 10.

The level of detail on the machine learning is not optimally depicted. The approach does not clearly show how to integrate data transformation steps, e.g. changing of a data type.

Future work consists of extending so to apply it for any domain.

\section{\cite{melchor_model-driven_2022}}
The approach shows an MDE method for formalizing machine learning, as well as the associated infrastructure in which the resulting tool will be deployed.

The approach introduced a comprehensive metamodel, but no concrete syntax.
The abstract syntax is defined using Eclipse Modeling Framework (EMF).
Arbitrary constraints can be modeled using OCL expressions.
Model transformations are not specified, yet.

Business understanding is not reflected in the approach.
Data understanding is partly given (Files are depicted but no details on the data features).
The loading of the data is described and the feature preparation, too.

However, as of now, details on the implementation are missing. Maybe they will come up in the near future since the publication is quite recent.

\section{\cite{moin_model-driven_2022}}
In~\cite{moin_model-driven_2022}, a textual modeling approach based on the ThingML framework intended to support the development of IoT devices with the extension of data analytics and machine learning is proposed. The ThingML framework supports the definition of software parts and components aligned with the UML standard. The communication between the components (things) is defined using ports, messages and state machines. The comprehensive approach, called ThingML+, extends the domain-specific language ThingML by adding means to enable data analytics and machine learning modeling during the modeling process. Theoretically, the framework can support any ML algorithm's implementation. Although the approach mainly focuses on the supervised ML algorithms, there are also templates for implementing unsupervised learning in the Github repository\footnote{\url{https://github.com/arminmoin/ML-Quadrat}}. The result of the modeling is transformed using model-to-code transformation to derive Java and Xtend\footnote{\url{https://www.eclipse.org/Xtext/}} code. 

From an language engineering perspective, the approach introduces each domain.
However, the modeling of constraints is not given, yet.

With the approach, business and data understanding is not fostered.
However, the implementation stack from data ingestion until the evaluation is presented.

The artifacts of the approach are presented.

\section{\cite{taibi_towards_2022}}
The approach introduces a DSL for AI formalization based on Sirius, a DSL development engine by Eclipse.

The metamodel is given in a online resource.
The concrete and abstract syntax is specified and given by sirius.
Constraints are not mentioned and model transformation are actually not implemented but are planed in future work.

In the referenced metamodel, means to specify requirements are given.
The business and data understanding is fostered by the comprehensive integration.
The loading and processing of data is specified with data activities.

Although the approach introduces a MDE for AI, it lacks in model transformation so to derive machine learning code with the formalization.

\section{\cite{portugal_preliminary_2016}}
Survey -> exclude for and only include in snowballing.

\section{\cite{ries_mde_2021}}
In this approach, a model-based definition of requirements is introduced.

The approach contributes to data understanding of datasets.
The approach focuses on requirements engineering and therefore, other dimensions are not presented.

However, it seems to be to complex to be applied to an industrial use case with more complex datasets. Additionally, the time consuming definition and formalization does not directly contribute to a better solution. Although, it supports the quality assurance of the final product.

\section{\cite{zucker_arbiter_2020}}
The given approach describes a DSL that enables to describe transparency, fairness, accountability and reproducability of ethical machine learning datasets.
The approach introduces a syntax based on SQL.

The purpose of the DSL is to provide a ethical machine learning support.
It is not designed to formalize the entire machine learning pipeline.
The level of detail on the description of the ethical aspects is quite high-level.
Additionally, the model transformations are mentioned but not covered in this approach.
